Lieb-Thirring inequalities for the shifted Coulomb Hamiltonian

In this paper we prove sharp Lieb-Thirring (LT) inequalities for the family of shifted Coulomb Hamiltonians. More precisely, we prove the classical LT inequalities with the semi-classical constant for this family of operators in any dimension $d\geq 3$ and any $\gamma \geq 1$. We also prove that the semi-classical constant is never optimal for the Cwikel-Lieb-Rozenblum (CLR) inequalities for this family of operators in any dimension. In this case, we characterize the optimal constant as the minimum of a finite set and provide an asymptotic expansion as the dimension grows. Using the same method to prove the CLR inequalities for Coulomb, we obtain more information about the conjectured optimal constant in the CLR inequality for arbitrary potentials.

==> CLRconjecture.tex <==
\section{On the CLR conjecture}\label{sec:CLR conj}


\begin{proof}[Proof of Theorem~\ref{thm:CLRconjecture}] 

Let $A_d$ be the function given in \eqref{eq:ad}.
For $t\in \R \backslash \{ -1,-2,\dots, -d+1 \}$
the derivative of $A_d$ satisfies the identity $A'_d(t) = A_d(t) g_d(t)$ with 
\begin{align*}
    g_d(t)\coloneqq \frac{1-\frac{d}{2}}{t+\frac{d}{2}} - \frac{\frac{d}{2}}{t+\frac{d}{2}-1} + \sum_{k=1}^{d-1} \frac{1}{t+k}\,. 
\end{align*}
As $A_d$ is positive for $t\geq 0$, it suffices to study the behavior of $g_d$ for $t\geq 0$. For $d \leq 4$, it is immediate to see that $g_d \leq 0$ and therefore $A_d$ is decreasing, which completes the proof in this case. 

For $d \geq 5$, we divide the proof into two cases. First, we consider the case when $d$ is even. Later, we deal with the case when $d$ is odd. In the even case, the proof follows the exact same steps of the proof of Theorem~\ref{thm: CLR Coulomb}. For convenience of the reader, we sketch these steps below.

{\em Step 1: the case $d> 5$ even.} 
For $d$ even, we note that the poles of the first two terms also appear as poles within the sum term. 
Rewriting $g_d$ as a quotient of co-prime polynomials, we obtian 
\begin{align*}
    g_d(t) = \frac{p(t)}{q(t)}, 
\end{align*}
where  $ q(t) \coloneqq \prod_{k=1}^{d-1} (t+k) $ and $p(t)$ is a polynomial of order $d-3$  satisfying 
\begin{align}
p(t) = -\frac{d}{2} \left(t^{d-3} + \left(\frac{d^2}{3} -d+ \frac{2}{3}\right) t^{d-4} + \mathcal{O}(t^{d-5})\right). \label{eq:polynomialform}
\end{align}
Thus, $p$ (and consequently $g_d$) has at most $d-3$ zeros. 
Analysing the behavior of $g_d$ near its poles and using the intermediate value theorem, as we did in the proof of Theorem~\ref{thm: CLR Coulomb}, we conclude that $g_d$ has at least one zero in each of the intervals $(-k-1,-k)$ for $k\in \{1,...,d-2\}\setminus \{ d/2, d/2-2\}$, and at least one zero in the interval $(-1, +\infty)$. 
Therefore, $g_d$ (and consequently $p$) has exactly one zero of order one 
in each of the described intervals. 
Hence, $p(t)$ can be written as a product as follows
\begin{align}
    p(t) = -\frac{d}{2} (t-\tilde{t}_d)\prod_{ k=1, \, k \notin  \left\{\frac{d}{2},\frac{d}{2}-2 \right\} }^{d-2} (t+k+\varepsilon_k) , \label{eq:factorised_p_conjecture}
\end{align}
where $\tilde{t}_d$ is the unique zero in the interval $(-1,+\infty)$. 
Expanding the r.h.s. of \eqref{eq:factorised_p_conjecture} then yields 
\begin{align}
   p(t) = -\frac{d}{2} t^{d-3} + \frac{d}{2} \left(\tilde{t}_d - \sum_{ k=1, \, k \notin  \left\{\frac{d}{2},\frac{d}{2}-2 \right\} }^{d-2}  (k+\varepsilon_k)\right) t^{d-4} + \mathcal{O}(t^{d-5}) . \label{eq:fac_p_conj_expand}
\end{align}
By comparing the coefficient 
in front of $t^{d-4}$
in \eqref{eq:fac_p_conj_expand} with the corresponding 
one in~\eqref{eq:polynomialform} and using the estimates $0\leq  \varepsilon_k \leq  1$, we conclude that
\begin{align*}
   \frac{d^2}{6} - \frac{3d}{2} +\frac{7}{3} \leq \tilde{t}_d \leq \frac{d^2}{6} -\frac{d}{2} -\frac{5}{3},
\end{align*}
which is within the interval in Theorem~\ref{thm:CLRconjecture}.

{\em Step 2: the case $d\geq 5$ odd.} 
For $d$ odd, we can not apply the same argument because $g_d(t)$ has five consecutive poles with different sign, namely $\{-\frac{d+1}{2},-\frac{d}{2},-\frac{d-1}{2},-\frac{d}{2}+1,-\frac{d-3}{2}\}$, and therefore the counting poles argument does not add up. Hence, we shall first use a simple estimate to get rid of the middle pole $t = \{-\frac{d-1}{2}\}$, and then proceed as in the previous step. To this end, it is more convenient for calculations to work with the shifted function
\begin{align} \label{eq:def tilde gd}
	\tilde{g}_d(s) 
    \coloneqq 
    g_d\left(s-\frac{d-1}{2}\right) 
    = 
    \frac{1-\frac{d}{2}}{s+\frac{1}{2}} - \frac{\frac{d}{2}}{s-\frac{1}{2}} + \sum_{j= -\frac{d-3}{2}}^{j=\frac{d-1}{2}} \frac{1}{s+j} \, .
\end{align}
Note that it suffices to study the behaviour of the shifted function for $s\geq \frac{d-3}{2}$. Moreover, the set of poles of $\tilde{g}_d(s)$ is $P \coloneqq \{-\frac{d-1}{2}, -\frac{d-1}{2}+1,...,-1,-\frac12, 0, \frac12, 1, ..., \frac{d-3}{2}\}$, and the pole at $t = -\frac{d-1}{2}$ is now located at $s=0$. The simple estimate we use to get rid of this pole is the following
\begin{align}
    \frac{1-a_d}{s-\frac12} + \frac{a_d}{s+\frac12}  \leq \frac{1}{s} \leq \frac{1/2}{s-\frac12} + \frac{1/2}{s+\frac12}, \quad \mbox{for $s\geq \frac{d-3}{2}$,} \label{eq: funny est}
\end{align}
where $a_d \coloneqq \frac12 +\frac{1}{2(d-3)}$. 
Precisely, we note that by~\eqref{eq: funny est} we have
\begin{align} \label{eq:squeeze}
    h_{a_d}(s) 
    < \tilde{g}_d(s) <
    h_{1/2}(s) 
    \quad \text{for} \quad 
    s> \frac{d-3}{2},
\end{align}
where $h_a(s)$ is the function defined by
\begin{align*}
    h_a(s) 
    \coloneqq 
    \frac{1-\frac{d}{2}}{s+\frac12} - \frac{\frac{d}{2}}{s-\frac12}  + \frac{1-a}{s-\frac12} + \frac{a}{s+\frac12} + \sum_{\substack{k=-\frac{d-3}{2}, \,  k \neq 0}}^{\frac{d-1}{2}} \frac{1}{s+k}
    \quad \text{for }
    s \in (\mathbb{R} \backslash P)\cup \{0\}. 
\end{align*} 
We can now apply the "counting poles" argument to the function $h_a(s)$ for $0 \leq a\leq 1$ to show that $h_a(s)$ has a unique zero inside the interval $(\frac{d-3}{2},+\infty)$ and to localize this zero. More precisely, by following the arguments in the previous step, one can show that 
\begin{align}
    h_a(s) \geq 0 \quad \mbox{for} \quad s\leq \left(\frac{d-1}{2} + a\right)^{-1} \left( \frac{d^3-6d^2+11d-3}{12} - \frac{d-2}{2} a\right)\label{eq:lowerbound}
\end{align}
and
\begin{align}
    h_a(s) \leq 0 \quad \mbox{for} \quad s \geq \left(\frac{d-1}{2} + a\right)^{-1} \left( \frac{d^3-6d^2+11d-3}{12} - \frac{d-2}{2} a\right)+ d-3 . \label{eq:upperbound}
\end{align}
Hence, by setting~ $a = 1/2$ in~\eqref{eq:upperbound} and using~\eqref{eq:squeeze}, we find that
\begin{align*}
    \tilde{g}_d(s) < 0 \quad \mbox{for}\quad s \geq \frac{d^2}{6} - \frac53 + \frac{1}{2d}.
\end{align*}
Shifting back, $g_d(t) = \tilde{g}_d(t+\frac{d-1}{2})$, and using the trivial estimate $\frac{1}{2d} \leq \frac16$ we obtain
\begin{align}
    g_d(t) < 0 \quad \mbox{for}\quad t \geq \frac{d^2}{6} - \frac{d}{2}-1. \label{eq:upperbound2}
\end{align}
Similarly, by setting $a= a_d = \frac12 + \frac{1}{2(d-3)}$ in~\eqref{eq:lowerbound} and using~\eqref{eq:squeeze} we find
\begin{align*}
    \tilde{g}_d(s) > 0 \quad \mbox{for}\quad \frac{d-3}{2}< s \leq \frac{d^2}{6} - d + \frac76 + \frac{3d-10}{6(d^2-3d+1)}.
\end{align*}
Shifting back and using the trivial estimate $\frac{3d-10}{6(d^2-3d+1)} \geq 0$ (valid for $d\geq 4$) we get 
\begin{align}
    g_d(t) > 0 \quad \mbox{for}\quad -1 < t \leq  \frac{d^2}{6} - \frac{3d}{2} +\frac{5}{3}. \label{eq:lowerbound2}
\end{align}
In particular, any zeros of $g_d(t)$ for $t>-1$ are within the interval in Theorem~\ref{thm:CLRconjecture}. Together with~\eqref{eq:upperbound2} and~\eqref{eq:lowerbound2}, this implies that the maximum of $A_d(t)$ is achieved inside the desired interval.

{\em Step 3: proving the asymptotic expression \eqref{eq:CLRconjecture_expansion}.}
Let now $t\geq 0$. 
We note that
\begin{align*}
    \frac{A_d(t)}{Q_d(t)} = 
    \frac{(t+\frac{d-1}{2})^d}{(t+\frac{d}{2})^{\frac{d}{2}} 
    (t+ \frac{d}{2}-1)^{\frac{d}{2}}}
    =
    \left(1+\frac{1}{\left(2t+d-1\right)^2-1}\right)^{\frac{d}{2}}\,.
\end{align*}
Thus, one has $A_d(t)>Q_d(t)$. 
We know the maximizing points of both $Q_d$ and $A_d$ are contained 
within the interval $[d^2/6-3d/2,d^2/6]$. For such $t$
we see that 
\begin{align*}
    \log A_d(t) - \log Q_d(t) 
    = \frac{d}{2}\log  \left(1+\frac{1}{\left(2t+d-1\right)^2-1}\right)
    \leq  C d^{-3}\,,
    \quad t\in \left[\frac{d^2}{6}-\frac{3d}{2},\frac{d^2}{6}\right]\,,
\end{align*}
with some uniform $C>0$ for sufficiently large $d$. This implies the first equality in \eqref{eq:CLRconjecture_expansion}. 
The second equality in \eqref{eq:CLRconjecture_expansion} follows from the expansion from Proposition~\ref{cor:asymptotic}.
\end{proof}
